Advanced Mapping Robot and High-Resolution Dataset

This paper presents a fully hardware synchronized mapping robot with support for a hardware synchronized external tracking system, for super-precise timing and localization. Nine high-resolution cameras and two 32-beam 3D Lidars were used along with a professional, static 3D scanner for ground truth map collection. With all the sensors calibrated on the mapping robot, three datasets are collected to evaluate the performance of mapping algorithms within a room and between rooms. Based on these datasets we generate maps and trajectory data, which is then fed into evaluation algorithms. We provide the datasets for download and the mapping and evaluation procedures are made in a very easily reproducible manner for maximum comparability. We have also conducted a survey on available robotics-related datasets and compiled a big table with those datasets and a number of properties of them.

==> sections/acknowledgement.tex <==
\section{Acknowledgement}
\label{sec:cknowledgement}

==> sections/experiment_calibrate.tex <==




\subsection{Motion Compensation}

\subsection{Odometry, IMU, EKF}

\subsection{Sensor data filtering}

Reflection, glass, removal of dynamic obstacles, 

\subsection{Range SLAM}

\subsection{Visual SLAM}


\subsection{Offline 3D Modelling (range)}

\subsection{Offline 3D Modeling vision - bundle adjustment - monocular)}

\subsection{Offline 3D Modeling vision - bundle adjustment - stereo)}

multiple stereo cameras at the same time!?

\subsection{Offline 3D Modelling combined)}

\section{Experiments}

Share bagfiles, CAD drawings, source code, Image (Docker), Video of the robot running...

\subsection{Bag files}

\subsubsection{SIST building number 1}
\subsubsection{parking garage}
\subsubsection{some other nice indoor building}


\subsubsection{ShanghaiTech Campus}


\subsubsection{Some nice city scene / architecutre}

\subsubsection{Some OLD/ historic city scene architecutre (archeology - Indiana Jones - Lara Croft)}

\subsubsection{Some nice nature}

\subsubsection{one more to have eight}


\subsection{Comparison of SLAM and Bundle adjustment systems}





==> sections/related_work.tex <==
\section{Related Works}
ICL-NUIM dataset \cite{ICL-NUIM} mainly focused on RGB-D camera with handheld perspective within simulated indoor environments. The ground truth of this dataset comes from the model of the room. 
Robot@Home dataset \cite{Robot@Home} consists of the data stream comes from 4 RGB-D camera and 2 2D Lidar, but there is no pose ground truth. % But it is said to have pose ground truth via algorithm in the table?! 
TUM-RGBD dataset \cite{TUM-RGBD}, as another indoor dataset, is captured by a synchronized Microsoft Kinect RGB-D camera both handheld and onboard of a ground robot. It has pose ground truth coming from a motion capture system at 100Hz. The images are with $640\times 480@30$Hz. 
EuRoC dataset\cite{EuRoC} is from a micro aerial vehicle (MAV). It is equipped with synchronized stereo monochrome cameras at 20 fps, inertia measurement unit (IMU) and has pose ground truth from laser tracking systems.
KITTI dataset\cite{KITTI}, as one of the most famous dataset regarding on autonomous driving, is equipped with a HDL-64E 3D Lidar, grayscale and RGB stereo cameras. All the Lidar and the cameras are synchronized and generates data at 10Hz. Global positioning system (GPS) and IMU data are also included in this dataset with 100Hz. The synchronization between GPS and IMU is not hardware-level synchronized with the camera or the Lidar. They use the time stamp to synchronize among them. 
Zurich Urban MAV dataset \cite{Zurich_Urban_MAV} is also based on MAVs. Different from EuRoC, it is recorded in outdoor environments. This capture system has barometer, gyrometer, accelerometer and GPS receiver synchronized with autopilot board and the cameras. Unlike EuRoC, its ground truth comes from algorithms instead of directly from the capture system. GPS location is only used for initial position in its ground truth pose calculation algorithm.
CoRBS dataset\cite{CoRBS} is the first to have ground truth of camera trajectory and 3D model of the scenes. The camera is also upgraded to Microsoft Kinect v2 compared to TUM-RGBD dataset launched in 2012. The RGB resolution is $1920\times 1080@$30Hz and the depth cloud also revolves at 30Hz and have $512\times 424$ pixels in each frame. The tracking system generates 3D pose ground truth at 120Hz with error of 0.39mm.
Oxford RobotCar dataset\cite{RobotCar} is a dataset with four types of heterogeneous sensors mounted on a ground vehicle. Its video stream consists of a stereo camera with three lens, three monocular RGB cameras. It obtains depth data through two 2D Lidar and a four-beam 3D Lidar. The platform is also equipped with a 6 degree of freedom (DOF) IMU and GPS/GLONASS system reports its position at 50Hz. The three monocular cameras are synchronized at 11.1Hz frame rate, as the stereo camera produces 16Hz. The Lidar scans at 12.5Hz. All these sensors have their clock calibrated using TICSync. 

\begin{thebibliography}{00}
\bibitem{ICL-NUIM} A. Handa, T. Whelan, J. McDonald, and A. J. Davison. A Benchmark for RGB-D Visual Odometry, 3D Reconstruction and SLAM. In Proceedings of the IEEE International Conference on Robotics and Automation (ICRA), pages 1524–1531. IEEE, 2014
\bibitem{Robot@Home} Ruiz-Sarmiento, J. R., Cipriano Galindo, and J. González-Jiménez. "Robot@ home, a robotic dataset for semantic mapping of home environments." The International Journal of Robotics Research 36.2 (2017): 131-141.
\bibitem{TUM-RGBD} J. Sturm, N. Engelhard, F. Endres, W. Burgard, and D. Cremers. A Benchmark for the Evaluation of RGB-D SLAM Systems. In Proceedings of the IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), pages 573–580. IEEE, 2012
\bibitem{EuRoC} M. Burri, J. Nikolic, P. Gohl, T. Schneider, J. Rehder, S. Omari, M. W. Achtelik, and R. Siegwart. The EuRoC Micro Aerial Vehicle Datasets. The International Journal of Robotics Research (IJRR), 2016.
\bibitem{KITTI} A. Geiger, P. Lenz, C. Stiller, and R. Urtasun. Vision Meets Robotics: The KITTI Dataset. The International Journal of Robotics Research (IJRR), 32(11):1231–1237, 2013
\bibitem{Zurich_Urban_MAV} Andras Majdik and Charles Till and Davide Scaramuzza. The Zurich urban micro aerial vehicle dataset. The International Journal of Robotics Research (IJRR) 36 (2017): 269-273
\bibitem{TMU-VI} Schubert, David, et al. "The TUM VI Benchmark for Evaluating Visual-Inertial Odometry." arXiv preprint arXiv:1804.06120 (2018).
\bibitem{ADVIO} Cortés, S., Solin, A., Rahtu, E., \& Kannala, J. (2018). ADVIO: An authentic dataset for visual-inertial odometry. In Proceedings of the European Conference on Computer Vision (ECCV) (pp. 419-434).
\bibitem{CoRBS} O. Wasenmuller, M. Meyer, and D. Stricker. CoRBS: Comprehensive RGB-D benchmark for SLAM using Kinect v2. In IEEE Winter Conference on Applications of Computer Vision (WACV), pages 1–7. IEEE, 2016
\bibitem{RobotCar} Maddern, Will, et al. "1 year, 1000 km: The Oxford RobotCar dataset." The International Journal of Robotics Research (2016): 0278364916679498. 


\end{thebibliography}


